Neuroadaptive Haptics: Comparing Reinforcement Learning from Explicit Ratings and Neural Signals for Adaptive XR Systems

Neuroadaptive haptics offers a path to more immersive extended reality (XR) experiences by dynamically tuning multisensory feedback to user preferences. We present a neuroadaptive haptics system that adapts XR feedback through reinforcement learning (RL) from explicit user ratings and brain-decoded neural signals. In a user study, participants interacted with virtual objects in VR while Electroencephalography (EEG) data were recorded. An RL agent adjusted haptic feedback based either on explicit ratings or on outputs from a neural decoder. Results show that the RL agent's performance was comparable across feedback sources, suggesting that implicit neural feedback can effectively guide personalization without requiring active user input. The EEG-based neural decoder achieved a mean F1 score of 0.8, supporting reliable classification of user experience. These findings demonstrate the feasibility of combining brain-computer interfaces (BCI) and RL to autonomously adapt XR interactions, reducing cognitive load and enhancing immersion.

==> input/1_teaser_figure.tex <==

% This is what most people (90+%) will see from your paper!

% - [ ]  use hemingwayapp.com (+SEO if hardcore) to make figure captions super precise
% - [ ]  are all the axes labels readable, font size 10 or up
% - [ ]  check for missing information: give someone the figure with captions to someone neutral to check if everything is clear from the figure alone
% - [ ]  for digital version: what is alt-text of figure, i.e. when hovering with the mouse over the figure what text appears next to the cursor
% - [ ]  for accessibility: write figure caption for the blind
%     - [ ]  explain what the figure shows
%     - [ ]  refactor using hemingwayapp.com

\begin{teaserfigure}
  \includegraphics[width=\textwidth]{paper/input/img/teaser-placeholder.png}
  \caption{Placeholder figure, planned to use the image for a final teaser with some infographics to the right?.}
  \Description{}
  \label{fig:teaser}
\end{teaserfigure}
